AdaViewPlanner: Adapting Video Diffusion Models for Viewpoint Planning in 4D Scenes

Recent Text-to-Video (T2V) models have demonstrated powerful capability in visual simulation of real-world geometry and physical laws, indicating its potential as implicit world models. Inspired by this, we explore the feasibility of leveraging the video generation prior for viewpoint planning from given 4D scenes, since videos internally accompany dynamic scenes with natural viewpoints. To this end, we propose a two-stage paradigm to adapt pre-trained T2V models for viewpoint prediction, in a compatible manner. First, we inject the 4D scene representation into the pre-trained T2V model via an adaptive learning branch, where the 4D scene is viewpoint-agnostic and the conditional generated video embeds the viewpoints visually. Then, we formulate viewpoint extraction as a hybrid-condition guided camera extrinsic denoising process. Specifically, a camera extrinsic diffusion branch is further introduced onto the pre-trained T2V model, by taking the generated video and 4D scene as input. Experimental results show the superiority of our proposed method over existing competitors, and ablation studies validate the effectiveness of our key technical designs. To some extent, this work proves the potential of video generation models toward 4D interaction in real world.

==> tex/figures/loss.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/fig6.pdf}
    \caption{Comparison of training loss curves: Ours, DanceCam and Ours w/o Motion.}
    \label{fig:6}
\end{figure}


==> tex/figures/vis_3.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/fig5.pdf}
    \caption{(a) Compared with other methods, our model generates smoother and more diverse trajectories that better follow instructions, while also exhibiting a cinematographic style centered on human actions. (b) Columns 1–3 show the reprojection of 4D human skeletons by using estimated camera parameters, while Column 4 presents the rendered results in 3D space. \textit{w/o Motion} exhibits viewpoint errors, whereas \textit{Relative Cam} suffers from scale perception issues.}
    \label{fig:5}
\end{figure}

